Impulse response of bilinear systems based on Volterra series representation

This paper focuses on the systems theory of bilinear dynamical systems using the Volterra series representation. The main contributions are threefold. First, we gain an input-output representation in the frequency domain, where the Laplace transform of the kernels can indeed be interpreted as transfer functions. Then, we derive the response of bilinear systems to a nascent delta function in time domain, i.e. the impulse response of bilinear systems. Finally, we study the relationships between this novel impulse response and the well-known Volterra kernels and adjust those to be compatible to the impulse response.

==> setup/settings.tex <==
% ======================================================================
% SI units
% ======================================================================
% Setup locale (e.g. comma vs. dot etc.)
\SISetupLocale

\sisetup{
  detect-all            = true,
  per-mode              = symbol,
  binary-units          = true,
  retain-zero-exponent  = true,
  exponent-product      = \cdot,
}

% You can declare your units here:
% \DeclareSIUnit\pixel{\text{px}}
% ======================================================================


% ======================================================================
% hyperref
% ======================================================================
\hypersetup{
  pdffitwindow    = false, % do not fit window to page when opened
  pdfstartview    = {FitH}, % fit the width of the page to window
  pdftitle        = {\thesisTitle},
  pdfauthor       = {\thesisAuthor},
  pdfkeywords     = {\thesisTitle, %
                     \thesisAuthor, %
                     \thesisType, %
                     Technische Universität München, %
                     TUM, %
                     Chair of Automatic Control, %
                     Lehrstuhl für Regelungstechnik %
                    }, % add your own the keywords (if any)
  pdfnewwindow    = false, % do not open links in new window
  colorlinks      = false, % use boxed links
  allbordercolors = tum blue!20, % color of the link boxes
}
% ======================================================================


% ======================================================================
% acro
% ======================================================================
\acsetup{
  only-used = false, %
  hyperref = true, %
}
% ======================================================================


% ======================================================================
% algorithm2e
% ======================================================================
\SetAlFnt{\small} % set font size
\SetKwComment{Comment}{$\triangleright$\ }{} % triangle comment
% ======================================================================


% ======================================================================
% cleveref
% ======================================================================
\crefformat{equation}{{#2(#1)#3}}
\Crefformat{equation}{{#2(#1)#3}}
\crefname{chapter}{\S}{\S}
\crefname{section}{\S}{\S}
\crefname{subsection}{\S}{\S}
\crefname{appendix}{\S}{\S}
% ======================================================================


% ======================================================================
% Manual lengthes
% ======================================================================
\renewcommand{\arraystretch}{1.40}
\setlength\parindent{0pt}
\setlength{\parskip}{5pt}
\setlength{\textheight}{235mm}
% ======================================================================


% ======================================================================
% Set default paths
% ======================================================================
\graphicspath{{images/}}
% ======================================================================


% ======================================================================
% Header & footer style
% ======================================================================
\pagestyle{fancy}

% fancy style for twopage
\lhead[\fancyplain{}{\thepage}]{\fancyplain{}{\nouppercase{\rightmark}}}
\rhead[\fancyplain{}{\nouppercase{\leftmark}}]{\fancyplain{}{\thepage}}
\cfoot{}

% ======================================================================


% ======================================================================
% Manual penalties
% ======================================================================
\widowpenalty10000
\clubpenalty10000
\displaywidowpenalty10000
% ======================================================================

% ======================================================================
% Setup listings
% ======================================================================
\lstset{
  language          = Matlab, % primary code language
  basicstyle        = \scriptsize\ttfamily, % the size of the fonts that are used for the code
  keywordstyle      = \color{tum blue}\bfseries, % keyword style
  commentstyle      = \color{tum green}, % comment style
  stringstyle       = \color{tum orange}, % string literal style
  numbers           = left, % where to put the line-numbers
  numberstyle       = \tiny\color{gray}, % the style that is used for the line-numbers
  stepnumber        = 1, % number each line
  numbersep         = 5pt, % how far the line-numbers are from the code
  backgroundcolor   = \color{white}, % choose the background color.
  showspaces        = false, % show spaces adding particular underscores
  showstringspaces  = false, % underline spaces within strings
  showtabs          = false, % show tabs within strings adding particular underscores
  frame             = tb, % adds top and bottom lines around the code
  rulecolor         = \color{black}, % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. commens (green here))
  tabsize           = 2, % sets default tabsize to 2 spaces
  captionpos        = b, % sets the caption-position to bottom
  breaklines        = true, % sets automatic line breaking
  breakatwhitespace = false, % sets if automatic breaks should only happen at whitespace
  title             = \lstname, % show the filename of files included with \lstinputlisting; also try caption instead of title
  escapeinside      = {@*}{*@}, % if you want to add a comment within your code
  morekeywords      = {*,...} % if you want to add more keywords to the set
}
% ======================================================================


% ======================================================================
% Theorem-like environments
% ======================================================================
\renewcommand{\qedsymbol}{$\blacksquare$}

\declaretheorem[style=plain, title=\nameThTheorem, numberwithin=chapter]{thm}
\declaretheorem[style=plain, title=\nameThLemma, numberwithin=chapter]{lem}
\declaretheorem[style=plain, title=\nameThProposition, numberwithin=chapter]{prp}
\declaretheorem[style=plain, title=\nameThCorollary, numberwithin=chapter]{cor}

\declaretheorem[style=remark, title=\nameThRemark, qed=$\vartriangle$, numberwithin=chapter]{rem}
\declaretheorem[style=remark, title=\nameThExample, qed=$\vartriangle$, numberwithin=chapter]{exa}

\declaretheorem[style=definition, title=\nameThDefinition, qed=$\blacktriangle$, numberwithin=chapter]{dfn}
% ======================================================================


% ======================================================================
% Equations highlighting (empheq)
% ======================================================================
\newcommand*\bluebox[1]{%
\colorbox{tum blue 1!10}{\hspace{1em}#1\hspace{1em}}}

\newcommand*\greenbox[1]{%
\colorbox{tum green!10}{\hspace{1em}#1\hspace{1em}}}

\newcommand*\orangebox[1]{%
\colorbox{tum orange!10}{\hspace{1em}#1\hspace{1em}}}
% ======================================================================


% ======================================================================
% Bibliography settings
% ======================================================================
\let\citePure\cite
\renewcommand{\cite}[2][]{\citet[#1]{#2}}
% ======================================================================

